Withdrawing the BGP Re-Routing Curtain: Understanding the Security Impact of BGP Poisoning via Real-World Measurements

The security of the Internet's routing infrastructure has underpinned much of the past two decades of distributed systems security research. However, the converse is increasingly true. Routing and path decisions are now important for the security properties of systems built on top of the Internet. In particular, BGP poisoning leverages the de facto routing protocol between Autonomous Systems (ASes) to maneuver the return paths of upstream networks onto previously unusable, new paths. These new paths can be used to avoid congestion, censors, geo-political boundaries, or any feature of the topology which can be expressed at an AS-level. Given the increase in BGP poisoning usage as a security primitive, we set out to evaluate poisoning feasibility in practice beyond simulation. To that end, using an Internet-scale measurement infrastructure, we capture and analyze over 1,400 instances of BGP poisoning across thousands of ASes as a mechanism to maneuver return paths of traffic. We analyze in detail the performance of steering paths, the graph-theoretic aspects of available paths, and re-evaluate simulated systems with this data. We find that the real-world evidence does not completely support the findings from simulated systems published in the literature. We also analyze filtering of BGP poisoning across types of ASes and ISP working groups. We explore the connectivity concerns when poisoning by reproducing a decade old experiment to uncover the current state of an Internet triple the size. We build predictive models for understanding an ASes' vulnerability to poisoning. Finally, an exhaustive measurement of an upper bound on the maximum path length of the Internet is presented, detailing how security research should react to ASes leveraging poisoned long paths. In total, our results and analysis expose the real-world impact of BGP poisoning on past and future security research.

==> related-work.tex <==
\section{Related Measurements}{\label{related-work}}

In the background on security impact, we covered relevant security literature. Here, we cover related Internet measurement research. LIFEGUARD from Katz-Bassett et al.~\cite{KatzBassett:2010wp,KatzBassett:2012gd} as well as Anwar et al.'s Interdomain Policy exploration~\cite{Anwar:2015tk} use algorithm similar to our \action methodology. They addressed steering return traffic around link failures between Amazon EC2 servers distributed between data centers. However, our algorithm explores greater depths in its breadth-first search of all possible paths from a single remote AS, rather than aggregating paths available from many poisoning ASes. While not directly related to our steering algorithm, work on BGP communities can influence inbound paths similarly to poisoning. Communities in the wild have been studied recently by Streibelt et al.~\cite{Streibelt:2018tp}. Outside of BGP, paths can be steered by other means, including the data-plane~\cite{Holterbach:2017gz} by SWIFT or newer, Internet architectures such as SCION~\cite{Perrig:2011tz}.
